Ozone: Efficient Execution with Zero Timing Leakage for Modern Microarchitectures

Time variation during program execution can leak sensitive information. Time variations due to program control flow and hardware resource contention have been used to steal encryption keys in cipher implementations such as AES and RSA. A number of approaches to mitigate timing-based side-channel attacks have been proposed including cache partitioning, control-flow obfuscation and injecting timing noise into the outputs of code. While these techniques make timing-based side-channel attacks more difficult, they do not eliminate the risks. Prior techniques are either too specific or too expensive, and all leave remnants of the original timing side channel for later attackers to attempt to exploit. In this work, we show that the state-of-the-art techniques in timing side-channel protection, which limit timing leakage but do not eliminate it, still have significant vulnerabilities to timing-based side-channel attacks. To provide a means for total protection from timing-based side-channel attacks, we develop Ozone, the first zero timing leakage execution resource for a modern microarchitecture. Code in Ozone execute under a special hardware thread that gains exclusive access to a single core's resources for a fixed (and limited) number of cycles during which it cannot be interrupted. Memory access under Ozone thread execution is limited to a fixed size uncached scratchpad memory, and all Ozone threads begin execution with a known fixed microarchitectural state. We evaluate Ozone using a number of security sensitive kernels that have previously been targets of timing side-channel attacks, and show that Ozone eliminates timing leakage with minimal performance overhead.

==> Related_work.tex <==
\section{Related Work}
In this section we review some of the previous works on both timing based side-channel attacks and mitigation techniques, giving emphasis to the mitigation techniques.

\subsection{Timing-based Side-channel Attacks}
The possibility of timing based side-channel attacks was first presented by  Kocher~\cite{Kocher}. Kocher showed that key dependent timing variations in modular exponentiation operations used in cryptographic algorithms like Diffie-Hellman and RSA can reveal encryption keys. Based on this work several implementations of timing-based side-channel attacks were presented~\cite{Dhem,Schindler} including remote timing attack on RSA~\cite{Brumley}. These attacks used variation in latency due to  program optimization as the basis for their attacks. 

Shortly after Kocher's attack, timing-based side-channel attacks based on cache contention were introduced. Early cache based timing side-channel attacks include~\cite{Bernstein,Osvik}. Cache-based timing attacks utilize time variation due to cache contention. Some cache-based timing side-channel attacks include L1 instruction cache based attacks~\cite{Aciicmez_rsa}, L1 data cache based attacks~\cite{Osvik,Zhang}, branch predictor cache based attacks~\cite{BranchP} and most recently last-level cache based attacks~\cite{LLC,Yarom}.

Timing-based side-channel attacks, like other types of side-channel attacks, mostly target cryptography algorithm implementations. Most commonly targeted implementations are RSA~\cite{Brumley,Dhem,Kocher,Schindler,Yarom,Yarom2} and AES~\cite{Bernstein,Bonneau,Gullasch,Tromer}, but attacks have been demonstrated on other algorithms such as the GDK keyboard key mapping function~\cite{Gruss}.  

\subsection{Timing-based Side-channel Mitigations}
There is a large body of work that has proposed various techniques to mitigate timing-based side-channel attacks. Here we discuss some of the proposed methods, categorizing them based on the sources of timing side-channels they target. 

%\paragraph{Control-flow-based timing side-channels:} 
Molnar {\em et. al} \cite{Molnar} presented the program counter transcript model that captures control-flow-based timing side-channels. The model assumes an adversary can observe the program counter value at each step of program execution. Based on this model, they propose a source-to-source code transformation where programs are modified to follow the same control path regardless of program inputs. After a transformed code is compiled, the generated machine code is verified to make sure it satisfies the program counter security model. We adopt a similar approach for control related timing channels, but unlike this earlier work, our work also eliminates cache and other resource contention based side channel attacks.
\ignore{This model fails to capture timing-based side-channel attacks that are based on hardware resource contention such as cache-timing side-channel attacks.}

Similarly, the work by Coppens {\em et. al}~\cite{Coppens} uses an if-conversion implemented at the back end of a compiler to eliminate
control-flow-based timing side-channels. They rely on the existence of cache partitioning or randomization techniques described in~\cite{Wang} to cope with cache-based side-channels. This work handles conditional stores by writing to dummy memory locations if a condition is not true. As stated by the authors, this approach creates complications while trying to determine the right dummy location. In addition to this, using dummy locations to handle conditional stores creates an additional side-channel. An attacker can infer whether a condition is true or not by looking at the memory location accessed through a cache side-channel attack.

The work of Wang {\em et. al} \cite{Wang} proposed two hardware-based approaches to mitigate cache-based side-channel attacks. The first approach allows applications to create private cache partitions by locking cache lines. The locked cache lines can not be evicted by other programs that do not own the cache lines. In the second approach, a Random Permutation Cache (RPcache) randomizes cache set mappings such that an attacker can not infer the cache lines that have been evicted. Kong et. al \cite{Kong} builds upon this work by using special load instructions to detect cache misses on critical data. Upon detection of a miss, all critical data is reloaded to cache to reduce secret data dependent time variations due to cache collisions. Parts of our approach are similar in that we lock down variables in the scratchpad. However, this earlier work does not account for control and microarchitectural timing variation, thus, programs in these earlier designs would still exhibit significant timing leakage.

Other approaches that uses existing hardware are proposed in \cite{Kim,cat}. These works targets last-level-cache-based side-channel attacks across virtual machines. In \cite{Kim} a set of last-level cache lines per core are locked to a virtual machine and are used by sensitive applications, like crypto algorithms. \ignore{The locking is achieved by setting aside memory pages called stealth pages at boot time and assigning them to each core. At run time, the hypervisor controls memory mappings such that the protected memory addresses are not evicted by an attacking virtual machine.} Similarly, \cite{cat} leverages Intel's Cache Allocation Technology (CAT) to partition the last-level cache into secure private regions for virtual machines. These approaches are only targeted at last-level-cache-based timing side-channels, thus, they are susceptible to the other types of control and microarchitetural side channels discussed above. \ignore{cache collisions that occur within the same process~\cite{ Bernstein,Bonneau} as well as control and microarchitetural side channels.} Ozone solves similar memory timing channels with the use of a scratchpad, and Ozone additionally addressed control flow and microarchitectural timing channels.

A recent and quite comprehensive effort by Braun {\em et. al} \cite{Braun} targets both control-flow and resource contention based side-channel attacks. They use time padding through delay loops to account for time variations due to different program path. The worst-case execution time is determined by dynamic profiling and is used for padding. They provide protection from cache-based timing side-channel attacks by reserving a core for the duration of execution of a sensitive function. This work has certain similarities with our work in that it applies side-channel protection on programmer annotated sensitive functions and reserves compute resources while the sensitive function is executing, but suffers from a number of shortcomings. First it doesn't guarantee fixed time execution like we do, as the pad time is an estimate. Furthermore, as we demonstrated in Section 2, even though a security sensitive function runs on a separate core, it is still subject to cache collision based attacks~\cite{Bonneau}. Finally, reserving resources comes at great cost. In order to prevent leakage through the last-level cache, last-level cache lines are reserved via page coloring. This requires disabling features like transparent huge pages and memory deduplication. Also, when a sensitive function is called all the process pages must be remapped to secure pages.

%Other more recent works target sensitive information leakage through memory access traces~\cite{Liu, Rane}. The side-channel information obtained by looking directly at memory access traces are similar to those obtained by timing-based side-channels, although the former provides fine grained information. Therefore it is important to look at the distinction of those works with ours. 
In Raccoon~\cite{Rane} the authors \ignore{note that all \textit{digital side-channels} are a result of variation in program execution and propose as a defense mechanism} propose obfuscation of program execution by executing extraneous program paths in addition to the real program path. The work is targeted at general programs and uses programmer annotation of secret variables and taint analysis to identify paths to obfuscate. We use similar concept as Raccoon to handle stores ({\em i.e.}, conditional store to a memory location is handled by first loading the data from the memory location, then based on the condition, storing a new value (the real path) or the old loaded value (decoy path). Beside targeting general programs, the main difference between Raccoon and this work is that Raccoon doesn't guarantee fixed-time execution and uses expensive software implementation of oblivious RAM (ORAM) to deal with leakage through data accesses ({\em e.g.}, cache-based timing side-channel attacks). Consequently, the runtime overheads are orders of magnitudes larger than those of Ozone.

Similarly Lui et. al \cite{Liu} propose a hardware-software mechanism to insure \textit{memory trace obliviousness} ({\em i.e.}, an attacker can not gain secret information using memory traces). \ignore{and at the same time reducing performance overhead by using compiler optimizations and a new type system to identify sensitive data dependent memory accesses.} Similar to Raccoon, GhostRider is targeted at general programs. GhostRider handles secret data dependent timing and address trace variation by padding either side of conditional branches. Non-memory access instructions are handled by padding the shortest path by NOP instructions. Memory access instructions are handled by actually executing the instructions on both paths. GhostRider uses instruction and data scratch pad memories with a deterministic processor to force determinism, but disallows concurrent execution of instructions as it requires determinism at the granularity of instructions. Like GhostRider, Ozone uses instruction and data scratchpad memory to prevent cache-contention-based side-channel attacks, but unlike Ghostrider, Ozone allows concurrent execution of instructions, which greatly improves performance as shown in Section 3.

Finally, mitigation by adding noise to measurements taken by attackers have been proposed \cite{Martin,Vattikonda,Zhang}. While these techniques have the potential to be near fixed latency, they are readily attacked with cache collision-based attacks~\cite{ Bernstein,Bonneau}.\ignore{, {\em e.g.}, aggressor shared cache attacks \cite{XXX} or microarchitectural initial state attacks \cite{XXX}. \tma{Need two more citations here, I believe these papers are already in the bib file.}}



